Spin-Dependent Signatures of Majorana Vortex Fusion within Planar Josephson Junctions

We investigate the magnetic characteristics and tunnelling signatures of a planar Josephson junction with Rashba spin-orbit coupling during the fusion of two Majorana vortices. By employing the topological phase diagram and conducting tight-binding simulations of the proposed device, we demonstrate that this fusion process induces a parity-dependent magnetic moment aligned with the junction axis. We further propose a method to probe the spin properties of the fusing Majorana zero modes through spin-resolved Andreev conductance measurements at the junction endpoints. To support our findings, we derive a low-energy effective Hamiltonian that provides a detailed microscopic description of the numerically observed phenomena. Our analysis enables the detection of Majorana fusion outcome from accessible spin current measurements, thus paving the way for future experimental verification and potential applications in topological quantum computation.

==> junk.tex <==
Line cut of Majorana zero mode probability densities through the normal region of the junction for different in-plane Zeeman field strengths. \textbf{(c)} Low energy spectrum as a function of $E_{z}$ for $\Phi = \Phi_{S}$. As $E_{z}$ is reduced, the two degenerate Majorana zero modes (purple) hybridize and split in energy.
